Gendered Mental Health Stigma in Masked Language Models

Mental health stigma prevents many individuals from receiving the appropriate care, and social psychology studies have shown that mental health tends to be overlooked in men. In this work, we investigate gendered mental health stigma in masked language models. In doing so, we operationalize mental health stigma by developing a framework grounded in psychology research: we use clinical psychology literature to curate prompts, then evaluate the models' propensity to generate gendered words. We find that masked language models capture societal stigma about gender in mental health: models are consistently more likely to predict female subjects than male in sentences about having a mental health condition (32% vs. 19%), and this disparity is exacerbated for sentences that indicate treatment-seeking behavior. Furthermore, we find that different models capture dimensions of stigma differently for men and women, associating stereotypes like anger, blame, and pity more with women with mental health conditions than with men. In showing the complex nuances of models' gendered mental health stigma, we demonstrate that context and overlapping dimensions of identity are important considerations when assessing computational models' social biases.

==> 08_Ethical_Considerations.tex <==
Our work has potential for positive impact in that it takes an initial step towards understanding gendered mental health stigma in mental health applications of language technologies. However, as prior NLP bias works have argued, we caution against using our method and/or tests as off-the-shelf metrics to evaluate models in practice.

% \subsection{Should NLP for Mental Health Applications Exist At All?}
% debatable lol


\subsection{Aggregation Metrics}
our methods aggregate scores for individual tests into more summarized metrics. Like Blodgett et al. criticized in the related works, aggregating metrics means that we are not separating scores for different subpopulations, and thus there may be additional differences in model behavior for subpopulations that we are not accounting for. For example, our tests do not tell us whether the model behaves differently for different races or different socioeconomic classes, though our methodology could be easily extended to incorporate more axes of demographic information. 

\subsection{Misuse Risk}

Critically, we intend this work to be a preliminary exploration of gendered mental health stigma, not a benchmark to evaluate models. We do not draw conclusions about which models may be better or worse, neither in general nor for specific applications, for a number of reasons. First, our tests are synthetic: the sentences we have hand-crafted may only represent a subset of how these language models actually get used in the real world. Furthermore, we do not explore what concrete impacts (if any) these model behaviors might have in downstream applications. Additional research is needed to measure these impacts, their actual harmfulness in the lived experiences of affected members of society, and the tradeoffs involved in different applications in order to determine what models can and should be used for specific applications.

Thus, our methodology should not be used as a metric to evaluate or select models in practice. Rather, we hope to provide useful insight into how gender plays into mental health stigma and how language models’ biases depend on specific social contexts like the mental health domain. 
